Robust Policy Optimization in Deep Reinforcement Learning

The policy gradient method enjoys the simplicity of the objective where the agent optimizes the cumulative reward directly. Moreover, in the continuous action domain, parameterized distribution of action distribution allows easy control of exploration, resulting from the variance of the representing distribution. Entropy can play an essential role in policy optimization by selecting the stochastic policy, which eventually helps better explore the environment in reinforcement learning (RL). However, the stochasticity often reduces as the training progresses; thus, the policy becomes less exploratory. Additionally, certain parametric distributions might only work for some environments and require extensive hyperparameter tuning. This paper aims to mitigate these issues. In particular, we propose an algorithm called Robust Policy Optimization (RPO), which leverages a perturbed distribution. We hypothesize that our method encourages high-entropy actions and provides a way to represent the action space better. We further provide empirical evidence to verify our hypothesis. We evaluated our methods on various continuous control tasks from DeepMind Control, OpenAI Gym, Pybullet, and IsaacGym. We observed that in many settings, RPO increases the policy entropy early in training and then maintains a certain level of entropy throughout the training period. Eventually, our agent RPO shows consistently improved performance compared to PPO and other techniques: entropy regularization, different distributions, and data augmentation. Furthermore, in several settings, our method stays robust in performance, while other baseline mechanisms fail to improve and even worsen the performance.

==> draft.tex <==

% related work

% Entropy in Policy Gradient \citep{williams1991function,ahmed2019understanding}. Entropy shows to improve performance \citep{mnih2016asynchronous,ahmed2019understanding}, smooth optimization landscape \citep{ahmed2019understanding}.

% More Stochastic policy-induced smoother optimization landscape and thus eventually helps to acheive better policy and high entropy might reduce the possible local optma \citep{ahmed2019understanding} , empirical finding, though they are environment-specific. 
% https://arxiv.org/pdf/1811.11214.pdf
% "The use of entropy maximization is designed to help keep the search alive by preventing convergence to a single choice of output, especially when several choices all lead to roughly the same reinforcement value"

% Work related to the use of Gaussian distribution as representing the continuous action.

% Work related to solving challenges of high-dimensional state and action spaces - data augmentation RAD DRAC

% Challenges in high-dimensional environments

% Exploration in On-policy policy gradient, use of entropy regularization
% Abstract
% add a start para of analyzing the effect of entropy and how that differs from existing findings, and then discuss our method and the results.
% Entropy has been shown important in RL training. However, properly setting the entropy might be important for RL task. In general, setup, the entropy starts high and gradually goes down as learning progresses. However, lower entropy and thus less exploratory policy can suffer from diverse data for the initial learning, and eventually, the policy can be converged into sub-optimal policy; this issue can even be severe in high-dimensional environments. In this paper, we explore the case where keeping a certain threshold of entropy throughout the training process can help better learning.
% In this paper, we propose a mechanism that encourages the agent to make high-entropy actions and thus potentially help in exploration throughout training in reinforcement learning (RL). First, we propose an action distribution by combining Gaussian and Uniform distribution in the continuous control tasks, which encourages higher entropic action than the standard Gaussian distribution. Then, we propose an RL algorithm Robust Policy Optimization (RPO), based on these techniques. We observe that RPO initially increases the policy entropy and then maintains a certain level of entropy throughout the training, which eventually results in a strong performance in many continuous control tasks. In experiments, we observe that data augmentation can boost the entropy of the policy. However, the performance improvement is not always consistent with the return performance, and sometimes the data augmentation can result in worsened performance.  We evaluated our methods on various continuous control tasks from DeepMind Control, OpenAI Gym, Pybullet, and IsaacGym. Empirically, our agent RPO shows improved performance compared to PPO and data augmentation-based method RAD and DRAC in several settings. In several settings, we observe that our method stays robust in performance while other baseline mechanisms fail to improve the base performance and even worsen the performance.





% Results on different DeepMind control environments are shown in Figures \ref{fig:return_fish_swim}, \ref{fig:return_hopper_hop}, \ref{fig:fish_swim_all}, \ref{fig:humanoid_run}, \ref{fig:return_quadruped_walk}, \ref{fig:return_quadruped_escape}, \ref{fig:return_walker_walk}, \ref{fig:return_pendulum_swingup}, \ref{fig:return_acrobot_swingup_sparse}, \ref{fig:return_dog_run_fetch}, \ref{fig:return_dog_stand_walk}
% here: Fish Swim in Figure \ref{fig:return_fish_swim}, Hopper Hop in Figure \ref{fig:return_hopper_hop}, 
% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.32\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/hopper_hop_train_return_rpo_ppo.png}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.32\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/hopper_hop_train_entropy_rpo_ppo.png}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.32\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/hopper_hop_train_policy_loss_rpo_ppo.png}
%   \end{minipage}
%   \hfill
%   \caption{RPO vs PPO Results on Deepmind Control Environments on Hopper Hop Environment.
%   }
%   \label{fig:return_hopper_hop}
% \end{figure}

% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.32\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/fish_swim_train_return_rpo_ppo.png}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.32\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/fish_swim_train_entropy_rpo_ppo.png}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.32\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/fish_swim_train_policy_loss_rpo_ppo.png}
%   \end{minipage}
%   \hfill
%   \caption{RPO vs PPO Results on Deepmind Control Environments on Fish Swim Environment.
%   }
%   \label{fig:return_fish_swim}
% \end{figure}

% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.32\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/hopper_hop_train_return_rpo.png}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.32\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/hopper_hop_train_entropy_rpo.png}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.32\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/hopper_hop_train_policy_loss_rpo.png}
%   \end{minipage}
%   \hfill
%   \caption{Comparison with PPO, RAD, and DRAC. Results on Deepmind Control Environments on Hopper Hop Environment.
%   }
%   \label{fig:return_hopper_hop}
% \end{figure}

% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.32\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/fish_swim_train_return_rpo.png}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.32\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/fish_swim_train_entropy_rpo.png}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.32\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/fish_swim_train_policy_loss_rpo.png}
%   \end{minipage}
%   \hfill
%   \caption{Comparison with PPO, RAD, and DRAC. Results on Deepmind Control Environments on Fish Swim Environment.
%   }
%   \label{fig:fish_swim_all}
% \end{figure}

% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/hopper_stand_train_return_ppo_rpo.png}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/hopper_hop_train_return_rpo_ppo.png}
%   \end{minipage}
%   \hfill
%   \caption{Results on Deepmind Control Environments
%   }
%   \label{fig:return1}
% \end{figure}

% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/humanoid_stand_train_return_ppo_rpo.png}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/humanoid_run_train_return_ppo_rpo.png}
%   \end{minipage}
%   \hfill
%   \caption{Results on Deepmind Control Environments
%   }
%   \label{fig:humanoid_run}
% \end{figure}

% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/humanoid_walk_train_return_ppo_rpo.png}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/quadruped_walk_train_return_ppo_rpo.png}
%   \end{minipage}
%   \hfill
%   \caption{Results on Deepmind Control Environments
%   }
%   \label{fig:return_quadruped_walk}
% \end{figure}

% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/quadruped_run_train_return_ppo_rpo.png}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/quadruped_escape_train_return_ppo_rpo.png}
%   \end{minipage}
%   \hfill
%   \caption{Results on Deepmind Control Environments
%   }
%   \label{fig:return_quadruped_escape}
% \end{figure}

% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/walker_stand_train_return_ppo_rpo.png}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/walker_walk_train_return_ppo_rpo.png}
%   \end{minipage}
%   \hfill
%   \caption{Results on Deepmind Control Environments
%   }
%   \label{fig:return_walker_walk}
% \end{figure}

% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/walker_run_train_return_ppo_rpo.png}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/pendulum_swingup_train_return_ppo_rpo.png}
%   \end{minipage}
%   \hfill
%   \caption{Results on Deepmind Control Environments
%   }
%   \label{fig:return_pendulum_swingup}
% \end{figure}

% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/acrobot_swingup_train_return_ppo_rpo.png}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/acrobot_swingup_sparse_train_return_ppo_rpo.png}
%   \end{minipage}
%   \hfill
%   \caption{Results on Deepmind Control Environments
%   }
%   \label{fig:return_acrobot_swingup_sparse}
% \end{figure}

% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/fish_swim_train_return_ppo_rpo.png}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/cheetah_run_train_return_ppo_rpo.png}
%   \end{minipage}
%   \hfill
%   \caption{Results on Deepmind Control Environments
%   }
%   \label{fig:return2}
% \end{figure}

% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/finger_spin_train_return_ppo_rpo.png}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/cartpole_balance_train_return_ppo_rpo.png}
%   \end{minipage}
%   \hfill
%   \caption{Results on Deepmind Control Environments
%   }
%   \label{fig:return2}
% \end{figure}

% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/dog_run_train_return_ppo_rpo.png}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/dog_fetch_train_return_ppo_rpo.png}
%   \end{minipage}
%   \hfill
%   \caption{Results on Deepmind Control Environments
%   }
%   \label{fig:return_dog_run_fetch}
% \end{figure}

% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/dog_stand_train_return_ppo_rpo.png}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/dog_walk_train_return_ppo_rpo.png}
%   \end{minipage}
%   \hfill
%   \caption{Results on Deepmind Control Environments
%   }
%   \label{fig:return_dog_stand_walk}
% \end{figure}


% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/dog_trot_train_return_ppo_rpo.png}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/swimmer_swimmer6_train_return_ppo_rpo.png}
%   \end{minipage}
%   \hfill
%   \caption{Results on Deepmind Control Environments
%   }
%   \label{fig:return2}
% \end{figure}

% \begin{figure}[!tbp]
%   \centering
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/cartpole_two_poles_train_return_ppo_rpo.png}
%   \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.49\columnwidth}
%     \includegraphics[width=0.99\textwidth]{figures/cartpole_three_poles_train_return_ppo_rpo.png}
%   \end{minipage}
%   \hfill
%   \caption{Results on Deepmind Control Environments
%   }
%   \label{fig:return2}
% \end{figure}

